A Message-Passing Interpretation of Adjoint Logic

We present a system of session types based on adjoint logic which generalize standard binary session types. Our system allows us to uniformly capture several new behaviors in the space of asynchronous message-passing communication, including multicast, where a process sends a single message to multiple clients, replicable services, which have multiple clients and replicate themselves on-demand to handle requests from those clients, and cancellation, where a process discards a channel without communicating along it. We provide session fidelity and deadlock-freedom results for this system, from which we then derive a logically justified form of garbage collection.

==> eptcsdata.tex <==
\providecommand{\firstpage}{60}
\providecommand{\publicationstatus}{F. Martins, D. Orchard (Eds.): Programming Language Approaches \\
to Concurrency- \& Communication-cEntric Software (PLACES 2019)\\
EPTCS 291, 2019, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.291.6}{10.4204/EPTCS.291.6}}

